Search for Baryon-Number-Violating Processes in $B^-$ Decays to the $\bar{\Xi}_{c}^{0} \bar{\Lambda}_{c}^{-}$ Final State

We report the results of the first search for $B^-$ decays to the $\bar{\Xi}_{c}^{0} \bar{\Lambda}_{c}^{-}$ final state using 711~${\rm fb^{-1}}$ of data collected at the $\Upsilon(4S)$ resonance with the Belle detector at the KEKB asymmetric-energy $e^+ e^-$ collider. The results are interpreted in terms of both direct baryon-number-violating $B^-$ decay and $\Xi_{c}^{0}-\bar{\Xi}_{c}^{0}$ oscillations which follow the Standard Model decay $B^- \to \Xi_{c}^{0} \bar{\Lambda}_{c}^{-}$. We observe no evidence for baryon number violation and set the 95\% confidence-level upper limits on the ratio of baryon-number-violating and Standard Model branching fractions ${\mathcal{B}(B^- \rightarrow \bar{\Xi}_{c}^{0} \bar{\Lambda}_{c}^{-})}/{\mathcal{B}(B^- \rightarrow \Xi_{c}^{0} \bar{\Lambda}_{c}^{-})}$ to be $< 2.7\%$ and on the $\Xi_{c}^{0} - \bar{\Xi}_{c}^{0}$ oscillation angular frequency $\omega$ to be $< 0.76\ \mathrm{ps}^{-1}$ (equivalent to $\tau_{\rm mix} > 1.3$~ps).

==> pub666-arxiv.tex <==
Belle Collaboration: T. Gu, V. Savinov, I. Adachi, H. Aihara, D. M. Asner, H. Atmacan, T. Aushev, R. Ayad, Sw. Banerjee, K. Belous, J. Bennett, M. Bessner, V. Bhardwaj, B. Bhuyan, D. Biswas, A. Bobrov, D. Bodrov, J. Borah, A. Bozek, M. Bra\v{c}ko, P. Branchini, T. E. Browder, A. Budano, M. Campajola, D. \v{C}ervenkov, M.-C. Chang, P. Chang, B. G. Cheon, K. Chilikin, K. Cho, S.-K. Choi, Y. Choi, S. Choudhury, S. Das, G. De Nardo, G. De Pietro, R. Dhamija, F. Di Capua, J. Dingfelder, Z. Dole\v{z}al, T. V. Dong, S. Dubey, P. Ecker, T. Ferber, D. Ferlewicz, B. G. Fulsom, V. Gaur, A. Giri, P. Goldenzweig, E. Graziani, Y. Guan, K. Gudkova, C. Hadjivasiliou, K. Hayasaka, H. Hayashii, M. T. Hedges, D. Herrmann, W.-S. Hou, C.-L. Hsu, N. Ipsita, A. Ishikawa, R. Itoh, M. Iwasaki, W. W. Jacobs, S. Jia, Y. Jin, K. K. Joo, T. Kawasaki, C. Kiesling, C. H. Kim, D. Y. Kim, K.-H. Kim, Y. J. Kim, P. Kody\v{s}, A. Korobov, S. Korpar, E. Kovalenko, P. Kri\v{z}an, P. Krokovny, T. Kuhr, K. Kumara, T. Kumita, Y.-J. Kwon, Y.-T. Lai, S. C. Lee, D. Levit, L. K. Li, Y. B. Li, L. Li Gioi, D. Liventsev, M. Masuda, T. Matsuda, S. K. Maurya, F. Meier, M. Merola, F. Metzner, K. Miyabayashi, R. Mizuk, G. B. Mohanty, R. Mussa, I. Nakamura, M. Nakao, Z. Natkaniec, A. Natochii, L. Nayak, M. Nayak, M. Niiyama, S. Nishida, S. Ogawa, G. Pakhlova, S. Pardi, H. Park, J. Park, S.-H. Park, A. Passeri, S. Patra, S. Paul, T. K. Pedlar, R. Pestotnik, L. E. Piilonen, T. Podobnik, E. Prencipe, M. T. Prim, M. R\"{o}hrken, G. Russo, S. Sandilya, L. Santelj, G. Schnell, C. Schwanda, Y. Seino, K. Senyo, M. E. Sevior, W. Shan, C. Sharma, J.-G. Shiu, E. Solovieva, M. Stari\v{c}, M. Takizawa, U. Tamponi, K. Tanida, F. Tenchini, R. Tiwary, K. Trabelsi, M. Uchida, Y. Unno, S. Uno, Y. Usov, S. E. Vahsen, K. E. Varvell, A. Vinokurova, E. Wang, M.-Z. Wang, X. L. Wang, S. Watanuki, E. Won, X. Xu, B. D. Yabsley, W. Yan, S. B. Yang, L. Yuan, Z. P. Zhang, V. Zhilich, V. Zhukova
